Benchmarking for Integrating Logic Rules with Everything Else

Integrating logic rules with other language features is increasingly sought after for advanced applications that require knowledge-base capabilities. To address this demand, increasingly more languages and extensions for such integration have been developed. How to evaluate such languages? This paper describes a set of programming and performance benchmarks for evaluating languages supporting integrated use of rules and other features, and the results of evaluating such an integrated language together with logic languages and languages not supporting logic rules.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{S. Costantini, E. Pontelli, A. Russo, F. Toni,\\R. Calegari, A. D'Avila Garcez, C. Dodaro, F. Fabiano,\\ S. Gaggl, A. Mileo, (Eds.): ICLP 2023\\
EPTCS 385, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.385.3}{10.4204/EPTCS.385.3}}

